Dynamic Frequency Assignment for Mobile Users in Multibeam Satellite Constellations

Mobile users such as airplanes or ships will constitute an important segment of the future satellite communications market. Operators are now able to leverage digital payloads that allow flexible resource allocation policies that are robust against dynamic user bases. One of the key problems is managing the frequency spectrum efficiently, which has not been sufficiently explored for mobile users. To address this gap, we propose a dynamic frequency management algorithm based on linear programming that assigns resources in scenarios with both fixed and mobile users by combining long-term planning with real-time operation. We propose different strategies divided into proactive strategies, which stem from robust optimization practices, and reactive strategies, which exploit a high degree of real-time control. This represents a tradeoff between how conservative long-time planning should be and how much real-time reconfiguration is needed. To assess the performance of our method and to determine which proactive and reactive strategies work better under which context, we simulate operational use cases of non-geostationary constellations with different levels of dimensionality and uncertainty, showing that our method is able to serve over 99.97\% of the fixed and mobile users in scenarios with more than 900 beams. Finally, we discuss the trade-offs between the studied strategies in terms of the number of served users, power consumption, and number of changes that need to happen during operations.

==> old_abstract.tex <==
The unprecedented levels of flexibility and scalability of the next generation of communication satellite systems call for new resource management algorithms that adapt to dynamic environments. The upcoming landscape of satellite communication services will be defined by an increased number of unique users, a large portion of which will correspond to mobile users such as planes or ships. The additional challenge introduced by these users is addressing the spatiotemporal uncertainty that comes in the form of delays, changes in their trajectory, or both. Given that mobile users will constitute an important segment of the market, satellite operators prioritize leveraging modern digital payloads to develop flexible resource allocation strategies that are robust against dynamic user bases.

One of the key problems in this context is managing the frequency spectrum efficiently. While numerous solutions address dynamic frequency assignment scenarios, the additional layer of complexity presented by mobile users has not been sufficiently studied, and it is unclear whether novel frequency assignment algorithms can address spatiotemporal uncertainty. Specifically, we argue that unexpected changes in the position of users introduce new restrictions into the frequency assignment, which previous algorithms in the literature might not be able to meet, especially if decisions need to be made in real-time and at scale.

To address this gap, we propose a dynamic frequency management algorithm based on linear programming that assigns resources in scenarios with both fixed and mobile users, accounting for the spatiotemporal uncertainty of the latter. Our method includes long-term planning and real-time operation, a synergy that has not been sufficiently explored for satellite communications and proves critical when operating under uncertainty. To fulfill the problem's scope, we propose different strategies that extend a state-of-the-art frequency management algorithm. These strategies are divided into proactive strategies, which stem from robust optimization practices, and reactive strategies, which exploit a high degree of real-time control.

To assess the performance of our algorithm and determine which strategies work better under which context, we simulate operational use cases of non-geostationary constellations with increasing levels of dimensionality and uncertainty. The results identify the strategies that best leverage the capabilities of satellite systems to allocate resources efficiently. We find that the studied strategies present several tradeoffs when addressing spatiotemporal uncertainty and analyze them in-depth. Finally, given the flexibility of our method, we discuss how additional constraints that are unique to certain constellations could be included in our formulation.

==> table_results_1.tex <==
\begin{table*}[t]
\small
    \centering
    \begin{tabular}{c|cc|cc|cc}
\hline
\rowcolor{lightbg}
$N_{users}=245$ & \multicolumn{2}{c}{Served users ($N_{served}/N_{users}$)} & \multicolumn{2}{c}{Power Consumption ($P/P^*$)} & \multicolumn{2}{c}{Reallocations ($N_{realloc}/N_{beams}$)} \\ \hline
\rowcolor{lightbg}
Config. & Low uncert. & High uncert. & Low uncert. & High uncert. & Low uncert. & High uncert. \\
\hline
$A$ & 0.998 (0.003) & 0.993 (0.005) & \textbf{0.996} (0.026) & \textbf{0.999} (0.027) & 0.092 (0.017) & 0.212 (0.015) \\
\hline
$B$ & 0.998 (0.003) & 0.997 (0.003) & 1.121 (0.034) & 1.107 (0.031) & 0.063 (0.013) & 0.159 (0.013) \\
\hline
$C$ & \textbf{1.000} (0.000) & 0.999 (0.002) & 1.138 (0.037) & 1.156 (0.055) & 0.063 (0.010) & 0.158 (0.014) \\
\hline
$D_1$ & 0.999 (0.002) & 0.997 (0.004) & 1.026 (0.020) & 1.093 (0.039) & 0.073 (0.009) & 0.180 (0.021) \\
$D_2$ & \textbf{1.000} (0.001) & \textbf{1.000} (0.001) & 1.085 (0.032) & 1.132 (0.060) & 0.079 (0.011) & 0.177 (0.016) \\
$D_3$ & \textbf{1.000} (0.000) & \textbf{1.000} (0.001) & 1.109 (0.030) & 1.197 (0.047) & 0.080 (0.012) & 0.191 (0.017) \\
$D_4$ & \textbf{1.000} (0.000) & \textbf{1.000} (0.000) & 1.160 (0.040) & 1.246 (0.045) & 0.084 (0.011) & 0.200 (0.019) \\
\hline
$E_1$ & 0.999 (0.002) & 0.994 (0.006) & 1.018 (0.024) & 1.019 (0.042) & 0.058 (0.009) & 0.180 (0.031) \\
$E_2$ & 0.999 (0.002) & 0.995 (0.005) & 1.043 (0.030) & 1.049 (0.046) & 0.050 (0.008) & 0.137 (0.011) \\
$E_3$ & \textbf{1.000} (0.001) & 0.999 (0.002) & 1.108 (0.047) & 1.092 (0.038) & \textbf{0.042} (0.006) & 0.084 (0.010) \\
\hline
$F_1$ & \textbf{1.000} (0.001) & 0.996 (0.004) & 1.011 (0.048) & 1.009 (0.063) & 0.059 (0.008) & 0.173 (0.020) \\
$F_2$ & \textbf{1.000} (0.001) & 0.997 (0.004) & 1.014 (0.041) & 1.028 (0.066) & 0.057 (0.011) & 0.138 (0.013) \\
$F_3$ & \textbf{1.000} (0.001) & 0.998 (0.003) & 1.052 (0.037) & 1.040 (0.058) & 0.043 (0.005) & 0.089 (0.012) \\
\hline
$G_1$ & 0.989 (0.005) & 0.992 (0.005) & 2.004 (0.172) & 1.964 (0.211) & 0.342 (0.017) & 0.369 (0.042) \\
$G_2$ & 0.987 (0.006) & 0.991 (0.006) & 2.014 (0.158) & 2.011 (0.224) & 0.350 (0.019) & 0.374 (0.042) \\
$G_3$ & 0.986 (0.005) & 0.990 (0.005) & 2.000 (0.149) & 1.968 (0.228) & 0.373 (0.021) & 0.391 (0.035) \\
\hline
$H_1$ & \textbf{1.000} (0.000) & 0.998 (0.002) & 1.059 (0.023) & 1.098 (0.033) & 0.053 (0.004) & 0.146 (0.008) \\
$H_2$ & \textbf{1.000} (0.000) & \textbf{1.000} (0.000) & 1.159 (0.040) & 1.175 (0.036) & 0.052 (0.007) & 0.116 (0.011) \\
$H_3$ & \textbf{1.000} (0.000) & \textbf{1.000} (0.000) & 1.250 (0.056) & 1.259 (0.046) & 0.043 (0.007) & \textbf{0.079} (0.011) \\
\hline
    \end{tabular}
    \caption{Results of the frequency assignment for two levels of uncertainty in a scenario with $N_{users}=245$, served by an average of 733 beams. The values in the table indicate the mean and standard deviation obtained from 10 runs. $P^*$ is defined as  the power consumption of a hypothetical case with no uncertainty.}
    \label{tab:results_1}
\end{table*}

==> table_strategies_2.tex <==
\begin{table*}[t!]
    \centering
    \footnotesize
    \begin{tabular}{lcccccccccccc}
        \hline
        \rowcolor{lightbg}
        Experiment config.
        & $A$   & $B$   & $C$
        & & $D_1$ & $D_2$ & $D_3$ & $D_4$
        & & $E_1$ & $E_2$ & $E_3$
        \\ 
        \hline
        \multirow{2}{*}{Proactive strat. (S1-S3)}
        & \multirow{2}{*}{--}
        & \multirow{2}{*}{--}
        & \multirow{2}{*}{--}
        & \multicolumn{1}{|c}{}
        & \multirow{2}{*}{--}
        & \multirow{2}{*}{--}
        & \multirow{2}{*}{--}
        & \multirow{2}{*}{--}
        & \multicolumn{1}{r}{$t_d=$} & $p_{50th}$ & $p_{75th}$ & $p_{95th}$ 
        \\
        & & & & & & & &
        & \multicolumn{1}{r}{$x_{min}=$} & 1.15 & 1.30 & 1.45
        \\ 
        \hline
        Reactive strat. (S4-S6)
        &  --
        & $x_{ch}=1$
        & $x_{slots}=1$
        & \multicolumn{1}{r}{$x_{spec}=$} & 0.05 & 0.10 & 0.15 & 0.20
        & & -- & -- & -- 
        \\
        \hline
    \end{tabular}
    \caption{Framework configurations consisting of proactive and reactive strategies, defined in Section \ref{sec:methods}. $p_{xth}$ indicates value of the x-th percentile of the delays and trajectory deviations of aeronautical mobile users.}
    \label{tab:configurations}
\end{table*}
